The CoSTAR Block Stacking Dataset: Learning with Workspace Constraints

A robot can now grasp an object more effectively than ever before, but once it has the object what happens next? We show that a mild relaxation of the task and workspace constraints implicit in existing object grasping datasets can cause neural network based grasping algorithms to fail on even a simple block stacking task when executed under more realistic circumstances. To address this, we introduce the JHU CoSTAR Block Stacking Dataset (BSD), where a robot interacts with 5.1 cm colored blocks to complete an order-fulfillment style block stacking task. It contains dynamic scenes and real time-series data in a less constrained environment than comparable datasets. There are nearly 12,000 stacking attempts and over 2 million frames of real data. We discuss the ways in which this dataset provides a valuable resource for a broad range of other topics of investigation. We find that hand-designed neural networks that work on prior datasets do not generalize to this task. Thus, to establish a baseline for this dataset, we demonstrate an automated search of neural network based models using a novel multiple-input HyperTree MetaModel, and find a final model which makes reasonable 3D pose predictions for grasping and stacking on our dataset. The CoSTAR BSD, code, and instructions are available at https://sites.google.com/site/costardataset.

==> ArXiV The CoSTAR Block Stacking Dataset_ Learning with Workspace Constraints (Version 21328)/arxiv_appendices.tex <==

\appendix


\subsection{Goals and Encoding Details, expanded}

Each successful stacking attempt consists of 5 sequential actions (Fig. \ref{fig:StackingSkillsNeuralNetwork}, \ref{fig:attempt}) out of the 41 possible object-specific actions described in Sec. \ref{ssec:datacollection}. 
Stacking attempts and individual actions vary in duration and both are divided into separate 100 ms time steps $t$ out of a total $T$. 
There is also a pose consisting of translation $v$ and rotation $r$ at each time step (Fig. \ref{fig:workspace}), which are encoded between [0,1] for use in a neural network as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\textbf{Translation $v$ vector encoding:}
%
\begin{equation}
v = (x, y, z)/d+0.5
\label{eq:translation_appendix}
\end{equation} 
% http://tex.stackexchange.com/a/95842/41590
% note: no empty newlines here, that will change indentation
\begin{conditions}
 d               & 4, max workspace diameter (meters) \\
 x,y,z           & robot base to gripper tip translation (meters) \\
 v               & array of 3 float values with range [0,1] \\
\end{conditions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Rotation $r$ axis-angle encoding:}
%
\begin{equation}
r  = (a_x, a_y, a_z, sin(\theta), cos(\theta))/s + 0.5
\label{eq:rotation_appendix}
\end{equation} 
% http://tex.stackexchange.com/a/95842/41590
% note: no empty newlines here, that will change indentation
\begin{conditions}
 a_x,a_y,a_z               & axis vector for gripper rotation \\
 \theta               & angle to rotate gripper (radians) \\
 s               & 1, scaling factor vs translation \\
 r               & array of 5 float values with range [0,1]
\end{conditions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\textbf{Example $E$ is the input to the neural network} defined at a single time step $t$ in a stacking attempt:
%
\begin{equation}
E_t = (I_0,I_t, v_t, r_t, a_t) 
\label{eq:example_appendix}
\end{equation} 
% http://tex.stackexchange.com/a/95842/41590
% note: no empty newlines here, that will change indentation
\begin{conditions}
 T               & Total time steps in one stack attempt \\
 t               & A single 100ms time step index in $T$ \\
 v_t             & Base to gripper translation, see Eq. \ref{eq:translation_appendix} \\
 r_t             & Base to gripper rotation, see Eq. \ref{eq:rotation_appendix} \\
 h, w, c         & Image height 224, width 224, channels 3\\
 \matrixdim{I}{h \times w \times c} & RGB image tensor scaled from -1 to 1 \\
 I_0             & First image, clear view of scene, $t=0$  \\
 I_t             & Current image, robot typically visible \\
 K, k            & 41 possible actions, 1 action's index \\
 \matrixdim{a_t}{1 \times K} & action one-hot encoding \\
%  a_t[k]          & 1 if an action is active, 0 otherwise \\
\end{conditions}


\noindent
\textbf{Ground Truth Goal Pose $G_t$} from Fig. \ref{fig:workspace} is the 3D pose time $g$ at which the gripper trigger to open or close, ending an action in a successful stacking attempt:
%
\begin{equation}
G_t = (v_g, r_g) | t \leq g \leq T, e_g \neq e_{g-1}, a_g == a_t
\label{eq:goal_appendix}
\end{equation} 
% http://tex.stackexchange.com/a/95842/41590
% note: no empty newlines here, that will change indentation
\begin{conditions}
  g  & First time the gripper moves after $t$ \\
  e  & gripper open/closed position in [0, 1] \\
  e_g \neq e_{g-1} & gripper position changed \\
  a_g == a_t & action at time $t$ matches action at time $g$ \\
  G_t & array of 8 float values with range [0,1] \\
  (v^g_t, r^g_t) & goal pose, same as $(v_g, r_g)$ \\
%   (v^p_t, r^p_t) & $P_t$ is a prediction of $G_t$ \\
\end{conditions}

\noindent
\textbf{Predicted Goal Pose $P_t = (v^p_t, r^p_t)$} is a prediction of $G_t$.

Each example $E_t$ has a separate sub-goal $G_t = (v^g_t, r^g_t)$ defined by (1) the current action $a_t$ and (2) the robot's 3D gripper pose relative to the robot base frame at the time step $t$ when the gripper begins moving to either grasp or release an object. Motion of the gripper also signals the end of the current action, excluding the final \texttt{move(home)} action, which has a fixed goal pose.
% The fixed final goal pose creates a complete task loop, thus it may be possible to simulate retries with the dataset.

\subsection{CoSTAR Block Stacking Dataset Details}

% If a sequence of actions is completed successfully without system errors and the traditional CoSTAR perception attempts to determines the height of the highest block, which indicates that a stack has been completed successfully. If successful, a file is saved indicating \texttt{success}, otherwise it is saved indicating \texttt{failure}. If any system errors occur, such as a security stop or motion planning failure, the example is saved as an \texttt{error.failure}.

We will outline a few additional CoSTAR BSD details here, and you can find our full documentation and links to both tensorflow and pytorch loading code at \url{sites.google.com/site/costardataset}. We include extensive notes with the dataset, explaining specific events and details of interest to researchers but outside the scope of this paper, such as where to obtain simulated robot models and dates when part failures occurred.
We have included certain details regarding the approach, data channels, update frequency, time synchronization, and problems encountered throughout the data collection process in Fig. \ref{table:dataset} that are not part of our approach to goal pose prediction, but may be useful for an approach to the stacking problem that is completely different from our own.
We have also tried to ensure sufficient data is available for tackling other perception and vision related challenges.
Attention to these details ensure a robotics dataset might prove useful as a benchmark for future research with methods that differ substantially from the original paper. 

In between stack attempts the robot returns to its past saved poses in an attempt to unstack the blocks to automatically reset itself for the next attempt. If too many sequential errors are encountered the data collection application restarts itself which mitigates most system state and traditional motion planning errors. With this approach we find that we can automate the collection of stack attempts with approximately 1 human intervention per hour due to incidents such as security stops and failure cases in which all objects remain exactly where they started. A successful stack attempt typically takes on average about 2 minutes to collect and contains about 18 seconds of data logged at 10 Hz (100ms time steps), but this figure varies substantially across examples.

The AR tags on the robot is used to perform dual quaternion hand-eye calibration before the dataset was collected, and the AR tag in the bin was used to initialize the table surface for data collection as described in~\cite{paxton2017costar}. 
Object models and AR tags are not utilized in the neural network.

\begin{figure*}[btp!]
\centering
\includegraphics[width=0.8\textwidth]{semantic_rotation_regression.png}
% https://docs.google.com/spreadsheets/d/e/2PACX-1vRRPOWTGuMHP-KKTvvMP3-3TmBXdoTGnJFfKvdIDaSS0ZJT-zM0qejGwES5-mi5MmCN3pdr43hTsfKk/pubchart?oid=154282479&amp;format=interactive
\caption{\label{fig:trainingplot} Final training of the HyperTree rotation model in Table \ref{table:HyperParameters} and Fig. \ref{fig:accuracy3d}. Higher accuracy, lower error,  and lower loss is better. Training was restarted on epoch 238, with a corresponding increase in learning rate. The final result is average angular errors of $16.0\degree$(val) and $18.3\degree$(test) at epoch 411. The horizontal axis represents performance at each training epoch on a linear scale while the vertical axis is log scale.}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{HyperTree Optimizer, losses, metrics, and preprocessing}

HyperTree search repeatedly runs a sampling from 100 random architectures and then estimates 10 additional random architectures by optimizing the Expected Improvement (EI) in training loss with a predictive Sparse Gaussian Process Model (SGPM). 
These limits were chosen due to the practical tradeoff between processing time and memory utilization when evaluating the SGPM, since we found GPyOpt prediction time outstripped model evaluation time with large sample sizes.
During training we perform optimization with Stochastic Gradient Descent (SGD). We also evaluated the Adam optimizer but we found it converged to a solution less reliably. Mini-batches consist of a random example sampled at a random time step. Input to the network includes the initial image plus the image, encoded pose, and one-hot encoded action ID at the randomly chosen time step. The input gripper pose was encoded as described in Fig. \ref{fig:attempt} at that time step as an input to the network. The output of the neural network is a prediction of either the x, y, z coordinate at the goal time step encoded as $v^g_t$ (Eq. \ref{eq:translation_appendix}, \ref{eq:goal_appendix}), or the angle-axis encoded rotation $r^g_t$ (Eq. \ref{eq:rotation_appendix}, \ref{eq:goal_appendix}) at the goal time step $g$.

We initialize the network by loading the pretrained ImageNet weights when available, and otherwise weights are trained from scratch utilizing He et. al. initialization~\cite{2015heinitalization}.
During HyperTree architecture search, we evaluate each model after a single epoch of training, so we either utilize a fixed reasonable initial learning rate such as 1.0, and for longer final training runs we utilized either a triangular or exp\_range (gamma=0.999998) cyclical learning rate~\cite{2015clr} with a cycle period of 8 epochs, maximum of 2.0, and minimum of $10^{-5}$. 

Translation training is augmented with cutout~\cite{2017cutout} plus random input pose changes of up to 0.5cm and 5 degrees. Each colored block is a 5.1 cm cube. 
An example of training for the final rotation model is shown in Fig. \ref{fig:trainingplot}.

% \begin{figure}[bt!]
% \centering
% \includegraphics[width=\columnwidth]{semantic_translation_regression.pdf}
% \caption{\label{fig:trainingplot} Training progress of the best translation regression HyperTree model. Here we can see that (TODO: update figure and add brief summary)}
% \end{figure}

\subsection{HyperTree Search Heuristics}

We incorporated several heuristics to improve HyperTree search efficiency. We found that the best models would quickly make progress towards predicting goal poses, so if models did not improve beyond 1m accuracy within 300 batches, we would abort training of that model early. We also found that some generated models would stretch, but not break the limits of our hardware, leading to batches that can take up to a minute to run and a single epoch training time of several hours, so we incorporated slow model stopping where after 30 batches the average batch time took longer than 1 second we would abort the training run. In each case where the heuristic limits are triggered we return an infinite loss for that model to the Bayesian search algorithm.

\begin{figure*}[btp!]
\centering
\vspace{0.1cm}\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{2018-05-15-10-45-10_example000006_success_tiled.jpg}
\vspace{0.1cm}\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{2018-05-15-15-20-21_example000006_success_tiled.jpg}
\vspace{0.1cm}\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{2018-07-05-11-45-26_example000005_success_tiled.jpg}
\vspace{0.1cm}\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{2018-08-02-19-36-36_example000003_success_tiled.jpg}
\vspace{0.1cm}\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{2018-08-06-15-45-17_example000002_success_tiled.jpg}
\vspace{0.1cm}\vspace{0.1cm}
\includegraphics[width=1.0\textwidth]{2018-07-31-20-22-20_example000001_failure_tiled.jpg}

\caption{ Examples from the dataset from top to bottom with key time steps in each example from left to right. 
All rows except the bottom represent successful stacking attempts. Also see the description in Fig. \ref{fig:attempt}. 
Viewing video and other details is highly recommended, see \url{sites.google.com/site/costardataset}.
% \ref{fig:MotionNetwork}.
}
\label{fig:attempt_appendix}
\vspace{-0.4cm}
\end{figure*}

==> ArXiV The CoSTAR Block Stacking Dataset_ Learning with Workspace Constraints (Version 21328)/bib.tex <==
%% LaTeX2e file `bib'
%% generated by the `filecontents' environment
%% from source `main' on 2019/03/12.
%%


==> bib.tex <==
%% LaTeX2e file `bib'
%% generated by the `filecontents' environment
%% from source `main' on 2019/03/12.
%%

